Strong and Controllable Blind Image Decomposition

Blind image decomposition aims to decompose all components present in an image, typically used to restore a multi-degraded input image. While fully recovering the clean image is appealing, in some scenarios, users might want to retain certain degradations, such as watermarks, for copyright protection. To address this need, we add controllability to the blind image decomposition process, allowing users to enter which types of degradation to remove or retain. We design an architecture named controllable blind image decomposition network. Inserted in the middle of U-Net structure, our method first decomposes the input feature maps and then recombines them according to user instructions. Advantageously, this functionality is implemented at minimal computational cost: decomposition and recombination are all parameter-free. Experimentally, our system excels in blind image decomposition tasks and can outputs partially or fully restored images that well reflect user intentions. Furthermore, we evaluate and configure different options for the network structure and loss functions. This, combined with the proposed decomposition-and-recombination method, yields an efficient and competitive system for blind image decomposition, compared with current state-of-the-art methods.

==> figures/discussion/edge-case.tex <==
\begin{figure}[htb!]
    \begin{minipage}{0.6\linewidth}
    \centering
        \begin{minipage}[c]{0.35in}
            \hfill 
            \text{\scriptsize Input\;}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/1-i.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/2-i.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/cropped_3-i.png}
        \end{minipage}%

        
        \begin{minipage}[c]{0.35in}
            \hfill 
            \text{\scriptsize Ours\;}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/1-o.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/2-o.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/cropped_3-o.png}
        \end{minipage}%



        % 同上，为下一行的图像重复
        \begin{minipage}[c]{0.35in}
            \hfill 
            \text{\scriptsize GT\;}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/1-t.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/2-t.png}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \includegraphics[width=0.96\linewidth, height=0.48\linewidth]{figures/discussion/cropped_3-t.png}
        \end{minipage}%


        % 同上，为下一行的图像重复
        \begin{minipage}[c]{0.35in}
            \hfill 
            \text{\scriptsize \;}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \centering 
            \text{\scriptsize Wrong prompt (1)}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \centering 
            \text{\scriptsize Wrong prompt (2)}
        \end{minipage}%
        \begin{minipage}[c]{0.29\linewidth}
            \centering 
            \text{\scriptsize Prompt (3)}
        \end{minipage}%
    \end{minipage}

    %\vspace{-0.5em}
    \caption{\textbf{Qualitative results of Task II.C: Controllable BID experiment.} The inputs contain degradation of rain streak, snow and watermark. Prompt (1): keep rain streak, snow and haze; Prompt (2): remove the reflection and fence; Prompt (3): remove snow and watermark. Our method well executes these prompts.}
    \label{fig:edge}
\end{figure}

==> figures/task3-b/task3-b.tex <==
\begin{figure*}[ht!]
    \begin{minipage}{1\textwidth}
        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Scene Image\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-a.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-a.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-a.png}
        \end{minipage}%

        
        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Rain Streak\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-b.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-b.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-b.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Snow\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-c.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-c.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-c.png}
        \end{minipage}%

        
        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Haze\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-d.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-d.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-d.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Raindrop\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-e.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-e.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-e.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Flare\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-flare.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-flare.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-flare.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Shadow\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-shadow.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-shadow.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-shadow.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Fence\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-fence.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-fence.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-fence.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Reflection\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-reflect.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-reflect.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-reflect.png}
        \end{minipage}%

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small Watermark\;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/1-water.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/2-water.png}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \includegraphics[width=0.9in, height=0.9in]{project-report/template/figures/task3-b/0-water.png}
        \end{minipage}%
        

        \begin{minipage}[c]{0.65in}
            \hfill 
            \text{\small \;}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \centering 
            \text{\small BIDeN}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \centering 
            \text{\small CBDNet}
        \end{minipage}%
        \begin{minipage}[c]{0.92in}
            \centering 
            \text{\small GT}
        \end{minipage}%

    \end{minipage}

    
    \caption{Qualitative results of Task IV.B (Image restoration of unified degradation removal in driving). For the details of all cases, please refer to Table~\ref{tab:task3-a}.}
    \label{fig:task3-b-fig}
\end{figure*}

==> figures/task3-b/task3-mask2.tex <==
\begin{figure*}[!htbp]
\begin{minipage}[c]{1\linewidth} 
    \begin{minipage}[c]{0.65in}
        \hfill 
        \text{\small BIDeN\;}
    \end{minipage}%
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/1-fence.png}
  \end{minipage}
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/1-flare.png}
  \end{minipage} 
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/1-reflect.png}
  \end{minipage} 
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/1-shadow.png}
  \end{minipage}  
     \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/1-water.png}
  \end{minipage} 


    \begin{minipage}[c]{0.65in}
        \hfill 
        \text{\small Ours\;}
    \end{minipage}%
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/2-fence.png}
  \end{minipage}
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/2-flare.png}
  \end{minipage} 
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/2-reflect.png}
  \end{minipage} 
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/2-shadow.png}
  \end{minipage}  
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/2-water.png}
  \end{minipage}  


    \begin{minipage}[c]{0.65in}
        \hfill 
        \text{\small GT\;}
    \end{minipage}%
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/0-fence.png}
  \end{minipage}
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/0-flare.png}
  \end{minipage} 
  \begin{minipage}[c]{0.92in} 
    \centering 
    \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/0-reflect.png}
  \end{minipage} 
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/0-shadow.png}
  \end{minipage}  
      \begin{minipage}[c]{0.92in} 
    \centering 
        \includegraphics[width=0.9in, height=0.9in]{figures/task3-b/0-water.png}
  \end{minipage}  

    \begin{minipage}[c]{0.65in}
        \hfill 
        \text{\small \;}
    \end{minipage}%
\begin{minipage}[c]{0.92in} 
    \centering 
    \text{\small Fence}
  \end{minipage} 
    \begin{minipage}[c]{0.92in} 
    \centering 
      \text{\small Flare}
  \end{minipage}  
    \begin{minipage}[c]{0.92in} 
    \centering 
    \text{\small Reflection}
  \end{minipage} 
      \begin{minipage}[c]{0.92in} 
    \centering 
    \text{\small Shadow}
  \end{minipage} 
    \begin{minipage}[c]{0.92in} 
    \centering 
      \text{\small Watermark}
  \end{minipage}  
\end{minipage}  
  \caption{Qualitative results (part 2) of Task III.B (Degradation masks reconstruction of unified degradation removal in driving). The input images contains all nine degradations. GT means ground truth, which is the referenced image.}
  \label{fig:task3-b-2}
\end{figure*}

==> table/table-effiecient.tex <==
\begin{table}[!htbp]
  \centering
    \fontsize{8}{9}\selectfont
    \setlength{\tabcolsep}{4pt}
  \caption{Comparison on model efficiency. We employ two metrics for assessment: the number of parameters and FLOPS. Compared to previous methods, CPNet marks a significant efficiency enhancement. Our proposed approach advances this efficiency even further; it boasts a parameter count that is merely one-ninth of CPNet’s and a FLOPS rate that is one-third of CPNet’s, indicating a substantial leap forward in terms of computational economy.}
\vspace{-0.5em}
  \begin{tabular}{lccccc}
    \toprule
    Method &MPRNet &All-in-one &BIDeN &CPNet &Ours\\

    \midrule
    Params (M) & 21.15 & 44.26 & 38.61 & 11.30 & 1.26\\
    FLOPs (G) & 135 & 350 & 344 & 102 & 30\\
    \bottomrule
  \end{tabular}
  \label{tab:ef}
\vspace{-1em}
\end{table}

==> table/table-task1-b.tex <==
\begin{table}[!h]
\centering
\fontsize{8}{9}\selectfont
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{1.2} % Adjust the row height

\begin{tabular}{l|cc|cc|cc|cc}
\toprule
    &\multicolumn{2}{c|}{Rain streak}&\multicolumn{2}{c|}{Snow}&\multicolumn{2}{c|}{Haze}&\multicolumn{2}{c}{Raindrop}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &28.32 &0.815 &24.80 &0.670 &29.83 &\textbf{0.942} &21.47 &0.893\\
    \hline
    Ours &\textbf{29.68} &\textbf{0.818} &\textbf{27.02} &\textbf{0.800} &\textbf{30.93} &0.920 &\textbf{24.67} &\textbf{0.915}\\
    \bottomrule
  \end{tabular}

\caption{Quantitative results on Task I.B (Degradation mask reconstruction of real-scenerio deraining in driving). We evaluate the performance of reconstruction of Rain-streak, Snow, Haze and Raindrop in PSNR and SSIM under the case: rain-streak + snow + moderate haze + raindrop. The best performance is marked in bold.}
% BIDeN performs well in haze reconstruction. CBDNet exhibits comparable performance to BIDeN in haze reconstruction and demonstrates superior performance over BIDeN in the reconstruction of rain-streak, snow, and raindrop.
\label{tab:task1-b}
\end{table}

==> table/table-task3-b-part2.tex <==
\begin{table*}[htbp]
  \centering
	  \fontsize{8}{9}\selectfont
         \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results of Task III.B (Degradation masks reconstruction of unified degradation removal in driving). The input images contains all nine degradations. We employed the PSNR matrics and the SSIM matrics to evaluate the reconstruction performance of BIDeN and CBDNet on fence, flare, reflection, shadow and watermark. The best performances has been marked in bold, while the second performance being underlined.}
  \vspace{4mm}
  \begin{tabular}{lc|c|c|c|c|c}
    \toprule
    \multicolumn{1}{c}{Method} &\multicolumn{1}{c|}{Metric} & Fence &Flare &Reflection&Shadow&Watermark\\
    \midrule
    \raisebox{-1.0\height}{BIDeN} 
               & PSNR$\uparrow$ &20.82&18.11&23.62&21.15&26.34 \\
               & SSIM$\uparrow$ &0.306&0.898&0.845&\textbf{0.671}&0.965\\
    \hline
    \raisebox{-1.0\height}{Ours} 
            & PSNR$\uparrow$ & \textbf{31.98} & \textbf{34.05} & \textbf{26.38} & \textbf{24.66} & \textbf{33.24} \\
            & SSIM$\uparrow$ & \textbf{0.809} & \textbf{0.976} & \textbf{0.903} & 0.621 & \textbf{0.966} \\


    \bottomrule
  \end{tabular}
  \label{tab:task3-b-2}
\end{table*}

==> table/table-task4-control.tex <==
\begin{table*}[!htbp]
  \centering
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results of Task IV.B (Removing specific real-scenario degradation based on given prompt in driving). The input for Prompt (1) to (3) contain degradations of rain streak, snow, haze, and raindrop. The input images for Prompt (4) to (6) have all nine types of degradation. Prompt (1): Remove the haze and the raindrop; Prompt (2): Generate the foggy cityscape; Prompt (3): Retain the scene image and the snow; Prompt (4): Keep the background and weather; Prompt (5): Compose image with rain-streak and fence; Prompt (6): Restore scene, flare, shadow and reflection together.}
  \vspace{4mm}
  \begin{tabular}{lc|c|c|c|c|c|c}
    \toprule
    \multicolumn{1}{c}{Method} &\multicolumn{1}{c|}{Metric} & Prompt (1) & Prompt (2) & Prompt (3) & Prompt (4) & Prompt (5) & Prompt (6)\\
    \midrule
    \raisebox{-1.0\height}{CaBINet} 
            & PSNR$\uparrow$ & 33.65 & 30.28 & 29.46 & 29.40 & 25.13 & 22.28\\
            & SSIM$\uparrow$ & 0.949 & 0.965 & 0.920 & 0.944 & 0.884 & 0.844\\


    \bottomrule
  \end{tabular}
  \label{tab:4control}
\end{table*}

==> table/table-task4-mask-control.tex <==
\begin{table*}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results on Task IV}
  \vspace{4mm}
  \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
    \toprule
    &\multicolumn{2}{c|}{Rainstreak}&\multicolumn{2}{c|}{Snow}&\multicolumn{2}{c|}{Haze}&\multicolumn{2}{c|}{Raindrop}&\multicolumn{2}{c|}{Flare} &\multicolumn{2}{c}{Shadow}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &25.14 &0.477 &20.65 &0.310 &24.30 &0.861 &17.13 &0.550 &20.82 &0.306 &18.11 &0.898 \\
    \hline
    Ours &\textbf{27.77} &\textbf{0.755} &\textbf{24.93} &\textbf{0.716} &\textbf{26.25} &\textbf{0.863} &\textbf{20.64} &\textbf{0.768} &\textbf{31.49} &\textbf{0.822} &\textbf{28.43} &\textbf{0.936}
    \\
    \bottomrule
    &\multicolumn{2}{c|}{Fence}&\multicolumn{2}{c|}{Refelction}&\multicolumn{2}{c|}{Watermark}&\multicolumn{2}{c|}{Control1}&\multicolumn{2}{c|}{Control2} &\multicolumn{2}{c}{Control3}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &23.62 &0.845 &21.15 &\textbf{0.671} &26.34 &\textbf{0.965} &- &- &- &- &- &- \\
    \hline
    Ours &\textbf{26.79} &\textbf{0.906} &\textbf{24.07} &0.602 &\textbf{33.08} &0.949 &\textbf{29.17} &\textbf{0.945} &\textbf{25.10} &\textbf{0.887} &\textbf{21.95} &\textbf{0.840} \\
    \bottomrule
  \end{tabular}
  \label{tab:42}
\end{table*}

==> table/table-task4-mask.tex <==
\begin{table*}[!htbp]
  \centering
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Comparison on Task IV.A. (Unified real-scenario degradation removal and degradation masks generation in driving) between BIDeN and Ours. BIDeN shows comparable results on the reconstruction of shadow. In contrast, Ours is better at all other cases. The best performances are marked in bold.}
  \vspace{4mm}
  \begin{tabular}{lc|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{1}{c}{Method} &\multicolumn{1}{c|}{Metric} & Scene Image & Rain Streak & Snow & Haze & Raindrop & Fence &Flare &Reflection&Shadow&Watermark\\
    \midrule
    \raisebox{-1.0\height}{BIDeN} 
               & PSNR$\uparrow$ & 21.38 & 25.14 & 20.65 & 24.30 & 17.13 &20.82&18.11&23.62&21.15&26.34 \\
               & SSIM$\uparrow$ & 0.678 & 0.477 & 0.310 & 0.861 & 0.550&0.306&0.898&0.845&\textbf{0.671}&0.965\\
    \hline
    \raisebox{-1.0\height}{Ours} 
            & PSNR$\uparrow$ & \textbf{26.42} & \textbf{27.56} & \textbf{24.63} & \textbf{26.32} & \textbf{19.25} & \textbf{31.98} & \textbf{34.05} & \textbf{26.38} & \textbf{24.66} & \textbf{33.24} \\
            & SSIM$\uparrow$ & \textbf{0.867} & \textbf{0.741} & \textbf{0.702} & \textbf{0.866} & \textbf{0.723} & \textbf{0.809} & \textbf{0.976} & \textbf{0.903} & 0.621 & \textbf{0.966} \\


    \bottomrule
  \end{tabular}
  \label{tab:4mask}
\end{table*}

==> table/table_ablation.tex <==
\begin{table}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Ablation}
  \vspace{4mm}
  \begin{tabular}{lcc|c|c}
    \toprule
    Ablation&\multicolumn{2}{c|}{Case(6)}&Mask&Controllable\\
    & PSNR$\uparrow$ & SSIM$\uparrow$ & & \\

    \midrule
    baseline &29.19 &0.903 &- &-\\
    +loss  &31.23 &0.950 &- &-\\
    +E  &31.70 &0.953 &\checkmark &-\\
    \hline
    +R &\textbf{31.75} &\textbf{0.955} &\checkmark &\checkmark\\
    \bottomrule
  \end{tabular}
  \label{tab:ab}
\end{table}

==> table/table_task2a.tex <==
\begin{table*}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results on Task II.A in driving scenario. We evaluate the performance in Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity (SSIM) under 6 BID cases, which are (1): rain streak, (2): rain streak + snow, (3): rain streak + light haze, (4): rain streak + heavy haze, (5): rain streak + moderate haze + raindrop, (6) rain streak + snow + moderate haze + raindrop. The best performance under each case is marked in bold with the second performance underlined.}
  \vspace{4mm}
  \begin{tabular}{lcc|cc|cc|cc|cc|cc}
    \toprule
    Case&\multicolumn{2}{c|}{MPRNet}&\multicolumn{2}{c|}{Restormer}&\multicolumn{2}{c|}{All-in-one}&\multicolumn{2}{c|}{BIDeN}&\multicolumn{2}{c|}{CPNet} &\multicolumn{2}{c}{Ours}\\
    & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    (1) &33.39 &0.945 &\underline{37.87} &\underline{0.972} &32.38 &0.937 &30.89 &0.932 &33.95 &0.948 &\textbf{42.13} &\textbf{0.993} \\
    (2) &30.52 &0.909 &32.68 &0.919 &28.45 &0.892 &29.34 &0.899 &\underline{33.42} &\underline{0.937} &\textbf{37.19} &\textbf{0.981} \\
    (3) &23.98 &0.900 &32.10 &\underline{0.954} &27.14 &0.911 &28.62 &0.919 &\underline{32.99} &0.932 &\textbf{36.16} &\textbf{0.986} \\
    (4) &18.54 &0.829 &\underline{29.41} &\underline{0.924} &19.67 &0.865 &26.77 &0.891 &29.02 &0.908 &\textbf{33.27} &\textbf{0.975} \\
    (5) &21.18 &0.846 &29.03 &0.903 &24.23 &0.889 &27.11 &0.898 &\underline{30.07} &\underline{0.925} &\textbf{32.83} &\textbf{0.968} \\
    (6) &20.76 &0.812 &28.36 &0.863 &22.93 &0.846 &26.44 &0.870 &\underline{29.57} &\underline{0.914} &\textbf{31.75} &\textbf{0.955} \\
    \bottomrule
  \end{tabular}
  \label{tab:2a1}
\end{table*}

==> table/table_task2a_mask.tex <==
\begin{table*}[!htbp]
  \centering
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results of Task II.B. (1) and (2) indicate that models are trained under different settings. The best performances are marked in bold with the second performance underlined.}
  \vspace{4mm}

  % 开始第一个minipage
  \begin{minipage}{0.48\textwidth} % 使用适当的宽度，这里为文档宽度的一半
    \noindent
    \begin{tabular}{lc|c|c|c|c|c}
      \toprule
      \multicolumn{1}{c}{Method} &\multicolumn{1}{c|}{Metric} & Cityscape & Rain Streak & Snow & Haze & Raindrop\\
      \midrule
      \raisebox{-1.0\height}{BIDeN} 
                 & PSNR$\uparrow$ & 21.38 & 25.14 & 20.65 & 24.30 & 17.13  \\
                 & SSIM$\uparrow$ & 0.678 & 0.477 & 0.310 & 0.861 & 0.550\\
      \hline
      \raisebox{-1.0\height}{CaBINet} 
                 & PSNR$\uparrow$ & 26.42 & 27.56 & 24.63 & 26.32 & 19.25 \\
                 & SSIM$\uparrow$ & 0.867 & 0.741 & 0.702 & 0.866 & 0.723 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  \hfill % 在两个minipage之间添加空间
  % 开始第二个minipage
  \begin{minipage}{0.48\textwidth}
    \hfill
    \begin{tabular}{lc|c|c|c}
      \toprule
      \multicolumn{1}{c}{Method} &\multicolumn{1}{c|}{Metric} & Cityscape & Rain Streak & Snow \\
      \midrule
      \raisebox{-1.0\height}{BIDeN} 
                 & PSNR$\uparrow$ & 21.38 & 25.14 & 20.65\\
                 & SSIM$\uparrow$ & 0.678 & 0.477 & 0.310\\
      \hline
      \raisebox{-1.0\height}{Ours} 
                 & PSNR$\uparrow$ & 26.42 & 27.56 & 24.63 \\
                 & SSIM$\uparrow$ & 0.867 & 0.741 & 0.702 \\
      \bottomrule
    \end{tabular}
  \end{minipage}
  
  \label{tab:2amask}
\end{table*}


==> table/table_task2a_mask_control.tex <==
\begin{table*}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results on Task II.B}
  \vspace{4mm}
  \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
    \toprule
    &\multicolumn{2}{c|}{Rainstreak}&\multicolumn{2}{c|}{Snow}&\multicolumn{2}{c|}{Haze}&\multicolumn{2}{c|}{Raindrop}&\multicolumn{2}{c|}{Remove haze} &\multicolumn{2}{c}{Remove rain}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &28.32 &0.815 &24.80 &0.670 &29.83 &\textbf{0.942} &21.47 &0.893 &- &- &- &- \\
    \hline
    Ours &\textbf{29.85} &\textbf{0.826} &\textbf{27.15} &\textbf{0.810} &\textbf{30.84} &0.912 &\textbf{25.33} &\textbf{0.925} &\textbf{32.99} &\textbf{0.932} &\textbf{35.69} &\textbf{0.984} \\
    \bottomrule
  \end{tabular}
  \label{tab:2a2}
\end{table*}

==> table/table_task2b.tex <==
\begin{table*}[!htbp]
  \centering
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results of Task II.B. (1) and (2) indicate that models are trained under different settings. The best performances are marked in bold with the second performance underlined.}
  \vspace{4mm}
  \begin{tabular}{lc|c|c|c|c|c}
    \toprule
    \multicolumn{1}{c}{Case} &\multicolumn{1}{c|}{Metric} & Input & MPRNet & BIDeN & CPNet & Ours \\
    \midrule
    \raisebox{-1.0\height}{Rainstreak} 
               & BRISQUE$\downarrow$ & 27.82 & 28.66 & 26.57 & \underline{25.58} & \textbf{23.40} \\
               & NIQE$\downarrow$ & 4.87 & \textbf{4.10} & 4.33 & \underline{4.13} & 4.31\\
    \hline
    \raisebox{-1.0\height}{Raindrop} 
               & BRISQUE$\downarrow$ & 24.88 & 29.17 & 21.22 & \underline{20.16} & \textbf{19.64} \\
               & NIQE$\downarrow$ & 5.63 & 4.87 & \underline{4.72} & \textbf{4.50} & 4.80 \\
    \hline
    \raisebox{-1.0\height}{Snow} 
               & BRISQUE$\downarrow$ & 22.68 & 25.78 & 22.42 & \underline{21.88} & \textbf{19.31} \\
               & NIQE$\downarrow$ & 4.75 & 4.48 & \underline{4.31} & \textbf{4.16} & 4.54 \\

    \bottomrule
  \end{tabular}
  \label{tab:2b}
\end{table*}

==> table/table_task4.tex <==
\begin{table}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results on Task IV. in driving scenario. We evaluate the performance in Peak Signal-to-Noise Ratio (PSNR) and Structural Similarity (SSIM) under 6 BID cases, which are (1): rain streak, (2): rain streak + snow + moderate haze + raindrop, (3) BHJ, (4) FGI, (5) BCDEFGHIJ, (6) BCDEFGHIJ->BCDE, (7) BCDEFGHIJ->BHJ, (8) BCDEFGHIJ->FGI. The best performance under each case is marked in bold with the second performance underlined. BID 80 epochs, CIDER }
  \vspace{4mm}
  \begin{tabular}{lcc|cc}
    \toprule
    Case&\multicolumn{2}{c|}{BIDeN}&\multicolumn{2}{c}{Ours}\\
    & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    (1) &27.24 &0.844 &\textbf{39.87} &\textbf{0.987}\\
    (2) &24.10 &0.762 &\textbf{30.09} &\textbf{0.929}\\
    (3) &26.51 &0.819 &\textbf{36.09} &\textbf{0.971}\\
    (4) &24.20 &0.814 &\textbf{32.72} &\textbf{0.968}\\
    (5) &21.38 &0.678 &\textbf{26.30} &\textbf{0.866}\\
    \bottomrule
  \end{tabular}
  \label{tab:4}
\end{table}

==> table/table_task4_mask_control.tex <==
\begin{table*}[!htbp]
  \centering
  %\fontsize{7}{3}\selectfont
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.2}
  \caption{Quantitative results on Task IV}
  \vspace{4mm}
  \begin{tabular}{l|cc|cc|cc|cc|cc|cc}
    \toprule
    &\multicolumn{2}{c|}{Rainstreak}&\multicolumn{2}{c|}{Snow}&\multicolumn{2}{c|}{Haze}&\multicolumn{2}{c|}{Raindrop}&\multicolumn{2}{c|}{Flare} &\multicolumn{2}{c}{Shadow}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &25.14 &0.477 &20.65 &0.310 &24.30 &0.861 &17.13 &0.550 &20.82 &0.306 &18.11 &0.898 \\
    \hline
    Ours &\textbf{27.77} &\textbf{0.755} &\textbf{24.93} &\textbf{0.716} &\textbf{26.25} &\textbf{0.863} &\textbf{20.64} &\textbf{0.768} &\textbf{31.49} &\textbf{0.822} &\textbf{28.43} &\textbf{0.936}
    \\
    \bottomrule
    &\multicolumn{2}{c|}{Fence}&\multicolumn{2}{c|}{Refelction}&\multicolumn{2}{c|}{Watermark}&\multicolumn{2}{c|}{Control1}&\multicolumn{2}{c|}{Control2} &\multicolumn{2}{c}{Control3}\\
    Method& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\

    \midrule
    BIDeN &23.62 &0.845 &21.15 &\textbf{0.671} &26.34 &\textbf{0.965} &- &- &- &- &- &- \\
    \hline
    Ours &\textbf{26.79} &\textbf{0.906} &\textbf{24.07} &0.602 &\textbf{33.08} &0.949 &\textbf{29.17} &\textbf{0.945} &\textbf{25.10} &\textbf{0.887} &\textbf{21.95} &\textbf{0.840} \\
    \bottomrule
  \end{tabular}
  \label{tab:42}
\end{table*}
